Approximate unitary $t$-designs by short random quantum circuits using nearest-neighbor and long-range gates

We prove that $poly(t) \cdot n^{1/D}$-depth local random quantum circuits with two qudit nearest-neighbor gates on a $D$-dimensional lattice with n qudits are approximate $t$-designs in various measures. These include the "monomial" measure, meaning that the monomials of a random circuit from this family have expectation close to the value that would result from the Haar measure. Previously, the best bound was $poly(t)\cdot n$ due to Brandao-Harrow-Horodecki (BHH) for $D=1$. We also improve the "scrambling" and "decoupling" bounds for spatially local random circuits due to Brown and Fawzi. One consequence of our result is that assuming the polynomial hierarchy (PH) is infinite and that certain counting problems are $\#P$-hard on average, sampling within total variation distance from these circuits is hard for classical computers. Previously, exact sampling from the outputs of even constant-depth quantum circuits was known to be hard for classical computers under the assumption that PH is infinite. However, to show the hardness of approximate sampling using this strategy requires that the quantum circuits have a property called "anti-concentration", meaning roughly that the output has near-maximal entropy. Unitary 2-designs have the desired anti-concentration property. Thus our result improves the required depth for this level of anti-concentration from linear depth to a sub-linear value, depending on the geometry of the interactions. This is relevant to a recent proposal by the Google Quantum AI group to perform such a sampling task with 49 qubits on a two-dimensional lattice and confirms their conjecture that $O(\sqrt n)$ depth suffices for anti-concentration. We also prove that anti-concentration is possible in depth O(log(n) loglog(n)) using a different model.

==> New arXiv/Summary.tex <==
\begin{center}
%\begin{table}
\begin{tabular} 
%to 0.8\textwidth 
{ | c | c |}
 \hline
\textbf{Notation} & \textbf{Definition}\\
 \hline
 \hline
$\|\cdot \|_\diamond$ & super-operator diamond norm\\
\hline
$\|\cdot \|_p$ & matrix $p$-norm for $p \in [0, \infty]$\\
\hline
$\Haar$ & the Haar measure\\
\hline
$\Haar(S)$ & Haar measure on subset $S$ of qudits\\
\hline
$\Haar(i,j)$ & Haar measure on qudits $i$ and $j$\\
\hline
$r_{\alpha,i}$ & $i$-th row in the $\alpha$ direction\\
\hline 
$\text{Rows}(\alpha,n)$ & the collection of rows of a lattice (with $n$ points) in the $\alpha$ direction\\
\hline
$G^{(t)}_\mu$ & $t$-th order quasi-projector according to distribution $\mu$ over quantum circuits\\
\hline
$\braket{i,j| G^{(t)}_\mu|k,l}$ & balanced moment of order $t$ defined as $\E_{C\sim \mu} [C_{i_1, j_1} \ldots C_{i_t, j_t} C\ast_{i_1, j_1} \ldots C^\ast_{i_t, j_t}]$\\
\hline
$\text{Ch}[G^{(t)}_\mu]$ & moment super-operator corresponding to $G^{(t)}_\mu$ also equal to $\E_{C \sim \mu}  [\mathrm{ ad}_{C^{\tensor t}} ]$\\
\hline
$G^{(t)}_\Haar$ & Haar projector of order $t$\\
\hline
$G^{(t)}_{i,j}$ & Haar projector of order $t$ on qudit $i$ and $j$\\
\hline
$g_{\text{Rows}(\alpha,n)}$ &  one step of the random circuit applied in parallel to the rows in $\alpha$ direction\\
\hline
$g_{R} (g_C)$ &  one step of the random circuit applied in parallel to the rows (columns) of a $2$D lattice\\
\hline
$G_{\text{Rows}(\alpha,n)}$ &  Haar projector applied in parallel to the rows in $\alpha$ direction\\
\hline
$G_R(G_C)$ &  Haar projector applied in parallel to the rows (columns) of a $2$D lattice\\
\hline
$G_{\text{Planes}(\alpha)}$ & Haar projector applied in parallel to the plane that are perpendicular to the direction $\alpha$\\
\hline
$\text{Coll} (\cA)$ & collision probability from super-operator $\cA$\\
\hline
$\text{Coll}_s$ & the expected collision probability of a random circuit after $s$ steps \\
\hline
$\mu^{\lattice,n}_{D,c,s}$ & the distribution over $D$-dimensional random circuits with $n$ qidits and parameters $c,s$\\
\hline
$\mu^{\text{CG}}_{s}$ & the distribution over random circuits after application of $s$ random long range gates\\
\hline
${\tilde G}_{n,D,c}$ & same as $G^{(t)}_{\mu^{\lattice,n}_{D,c,s}}$ except that we replace $g^s_{\text{Rows} (\alpha,n)}$ with $G_{\text{Rows} (\alpha,n)}$.\\
\hline
${\hat G}_{n,D,c,s}$ & one block of ${\tilde G}_{n,D,c}$ defined as $G_{\text{Rows}(D,n)} \tilde{G}^{\tensor n^{1/D}}_{n^{1-1/D}, D-1, c,s} G_{\text{Rows}(D,n)}$.\\
\hline
\end{tabular}
%\caption{Summary of the notations and definitions used in this paper}
%\label{table:summary}
%\end{table}
\end{center}


==> New arXiv/circ1.tex <==
\begin{figure}
\begin{center}
\begin{tikzpicture}[thick,scale=0.4]
\foreach \y in {0,..., 5}{
\draw[blue] (0,\y) -- (1,\y); \draw[blue] (2,\y) -- (3,\y); \draw[blue] (4,\y) -- (5,\y); 
}
\foreach \x in {0,...,5}{
\foreach \y in {0,...,5}{
\fill[black] (\x,\y) circle (0.1);
}}

\foreach \x in {0,1,4,5}{
\foreach \y in {1,3,5}{
\fill[black] (\x,\y) circle (0.1);
}}
\foreach \y in {0,2,4}{
\fill[black] (2,\y) circle (0.1);
\fill[black] (3,\y) circle (0.1);
}

%\node[draw, thick] at (-3,2) {1};
\node[inner sep=0,anchor=east,text width=1cm] (note1) at (-3,2) {
   (1) };

\begin{scope}[xshift=20cm]

\foreach \y in {0,..., 5}{
\draw[blue] (1,\y) -- (2,\y); \draw[blue] (3,\y) -- (4,\y); 
}
\foreach \x in {0,...,5}{
\foreach \y in {0,...,5}{
\fill[black] (\x,\y) circle (0.1);
}}

\foreach \x in {0,1,4,5}{
\foreach \y in {1,3,5}{
\fill[black] (\x,\y) circle (0.1);
}}
\foreach \y in {0,2,4}{
\fill[black] (2,\y) circle (0.1);
\fill[black] (3,\y) circle (0.1);
}

\node[inner sep=0,anchor=east,text width=1cm] (note1) at (-3,2) {
   (2) };

\end{scope}
%\end{scope}
\end{tikzpicture}
\end{center}
%\caption{ The architecture proposed by the quantum-AI group at Google to
%  demonstrate quantum supremacy consists of a 2D lattice of
%  superconducting qubits.  This figure depicts two illustrative
%  timesteps in this proposal.  At each timestep, 2-qubit gates (blue)
%  are applied across some pairs of neighbouring qubits, and random
%  single-qubit gates (black) are applied on other
%  qubits.\label{fig:google}}
\end{figure}

\begin{figure}
\begin{center}
\begin{tikzpicture}[thick,scale=0.4]
\begin{scope}[rotate=90]

\foreach \y in {0,..., 5}{
\draw[blue] (0,\y) -- (1,\y); \draw[blue] (2,\y) -- (3,\y); \draw[blue] (4,\y) -- (5,\y); 
}

\foreach \x in {0,...,5}{
\foreach \y in {0,...,5}{
\fill [black] (\x,\y) circle (0.1);
}}


\foreach \x in {0,1,4,5}{
\foreach \y in {1,3,5}{
\fill[black] (\x,\y) circle (0.1);
}}
\foreach \y in {0,2,4}{
\fill[black] (2,\y) circle (0.1);
\fill[black] (3,\y) circle (0.1);
}


\node[inner sep=0,anchor=east,text width=1cm] (note1) at (2,8) {
   (3) };


\end{scope}


\begin{scope}[xshift=20cm]
\begin{scope}[rotate=90]

\foreach \y in {0,..., 5}{
\draw[blue] (1,\y) -- (2,\y); \draw[blue] (3,\y) -- (4,\y); 
}
\foreach \x in {0,...,5}{
\foreach \y in {0,...,5}{
\fill[black] (\x,\y) circle (0.1);
}}

\foreach \x in {0,1,4,5}{
\foreach \y in {1,3,5}{
\fill[black] (\x,\y) circle (0.1);
}}
\foreach \y in {0,2,4}{
\fill[black] (2,\y) circle (0.1);
\fill[black] (3,\y) circle (0.1);
}


\node[inner sep=0,anchor=east,text width=1cm] (note1) at (2,8) {
   (4) };

\end{scope}
\end{scope}
\end{tikzpicture}
\end{center}
\caption{ The random circuit model in definition \ref{def:modelsD}. Each black circle is a
  qudit and each blue link is a random $\text{SU}(d^2)$ gate. The model does $O(\sqrt n\poly(t))$
  rounds alternating between applying (1) and (2). Then for $O(\sqrt n\poly(t))$ rounds it
  alternates between (3)
  and then (4).  This entire loop is then repeated $O(\poly(t))$ times.
%, and random single-qubit gates (black) are applied on other   qubits.
\label{fig:ourmodels}}
%\caption{ For $O(\sqrt n)$ time first apply (1) and then (2) and then for $O(\sqrt n)$ time first apply (3) and then (4) and repeat this for $O(1)$ times.\label{fig:google}}
\end{figure}

==> New arXiv/circ2.tex <==
THIS FILE IS NO LONGER USED.  INSTEAD ITS BEEN MOVED TO CIRC1.TEX

\begin{figure}
\begin{center}
\begin{tikzpicture}[thick,scale=0.4]
\begin{scope}[rotate=90]

\foreach \y in {0,..., 5}{
\draw[blue] (0,\y) -- (1,\y); \draw[blue] (2,\y) -- (3,\y); \draw[blue] (4,\y) -- (5,\y); 
}

\foreach \x in {0,...,5}{
\foreach \y in {0,...,5}{
\fill [red] (\x,\y) circle (0.1);
}}


\foreach \x in {0,1,4,5}{
\foreach \y in {1,3,5}{
\fill[red] (\x,\y) circle (0.1);
}}
\foreach \y in {0,2,4}{
\fill[red] (2,\y) circle (0.1);
\fill[red] (3,\y) circle (0.1);
}


\node[inner sep=0,anchor=east,text width=1cm] (note1) at (2,8) {
   (2) };


\end{scope}


\begin{scope}[xshift=20cm]
\begin{scope}[rotate=90]

\foreach \y in {0,..., 5}{
\draw[blue] (1,\y) -- (2,\y); \draw[blue] (3,\y) -- (4,\y); 
}
\foreach \x in {0,...,5}{
\foreach \y in {0,...,5}{
\fill[red] (\x,\y) circle (0.1);
}}

\foreach \x in {0,1,4,5}{
\foreach \y in {1,3,5}{
\fill[red] (\x,\y) circle (0.1);
}}
\foreach \y in {0,2,4}{
\fill[red] (2,\y) circle (0.1);
\fill[red] (3,\y) circle (0.1);
}


\node[inner sep=0,anchor=east,text width=1cm] (note1) at (2,8) {
   (4) };

\end{scope}
\end{scope}
\end{tikzpicture}
\end{center}
\caption{ The random circuit model in definition \ref{def:modelsD}. Each red circle is a qudit and each blue link is a random $\text{SU}(d^2)$ gate. The model for $O(\sqrt n)$ first applies (1) and then (2). Then for $O(\sqrt n)$ first applies (3) and then (4), and continues these two steps for $O(1)$ rounds
%, and random single-qubit gates (red) are applied on other   qubits.
\label{fig:ourmodels}}
%\caption{ For $O(\sqrt n)$ time first apply (1) and then (2) and then for $O(\sqrt n)$ time first apply (3) and then (4) and repeat this for $O(1)$ times.\label{fig:google}}
\end{figure}

==> New arXiv/google_fig.tex <==
\begin{figure}[h]
\begin{center}
\begin{tikzpicture}[very thick,scale=0.7]
\draw[blue] (2,1) -- (3,1); \draw[blue] (2,3) -- (3,3); \draw[blue] (2,5) -- (3,5);
\draw[blue] (0,0) -- (1,0); \draw[blue] (0,2) -- (1,2); \draw[blue] (0,4) -- (1,4);
\draw[blue] (4,0) -- (5,0); \draw[blue] (4,2) -- (5,2); \draw[blue] (4,4) -- (5,4);
\foreach \x in {0,...,5}{
\foreach \y in {0,...,5}{
\fill (\x,\y) circle (0.1);
}}
\foreach \x in {0,1,4,5}{
\foreach \y in {1,3,5}{
\fill[black] (\x,\y) circle (0.1);
}}
\foreach \y in {0,2,4}{
\fill[black] (2,\y) circle (0.1);
\fill[black] (3,\y) circle (0.1);
}
\begin{scope}[xshift=15cm]
\begin{scope}[rotate=90]
\draw[blue] (2,1) -- (3,1); \draw[blue] (2,3) -- (3,3); \draw[blue] (2,5) -- (3,5);
\draw[blue] (0,0) -- (1,0); \draw[blue] (0,2) -- (1,2); \draw[blue] (0,4) -- (1,4);
\draw[blue] (4,0) -- (5,0); \draw[blue] (4,2) -- (5,2); \draw[blue] (4,4) -- (5,4);
\foreach \x in {0,...,5}{
\foreach \y in {0,...,5}{
\fill (\x,\y) circle (0.1);
}}
\foreach \x in {0,1,4,5}{
\foreach \y in {1,3,5}{
\fill[black] (\x,\y) circle (0.1);
}}
\foreach \y in {0,2,4}{
\fill[black] (2,\y) circle (0.1);
\fill[black] (3,\y) circle (0.1);
}
\end{scope}
\end{scope}
\end{tikzpicture}
\end{center}
\caption{ The architecture proposed by the quantum AI group at Google to
  demonstrate quantum supremacy consists of a 2D lattice of
  superconducting qubits.  This figure depicts two illustrative
  timesteps in this proposal.  At each timestep, 2-qubit gates (blue)
  are applied across some pairs of neighboring qubits.
%, and random single-qubit gates (red) are applied on other   qubits.
\label{fig:google}}
\end{figure}



==> New arXiv/macros.tex <==
\usepackage{amsmath, amsthm, amssymb,color,fullpage,url,booktabs,enumitem}  %cite
\urlstyle{sf}
\usepackage{graphicx}
\synctex=1

\usepackage{prettyref}
\newrefformat{cor}{Corollary~\ref{#1}}
\newrefformat{prop}{Proposition~\ref{#1}}
\input{restate.tex}

\ifdefined\blackandwhite
\usepackage[pdftex]{hyperref} %pagebackref
\else
\usepackage[colorlinks,pdftex]{hyperref} %pagebackref
\hypersetup{citecolor = blue, linkcolor = red!70!black}
\fi

\usepackage{braket}
\usepackage{mathtools}
\usepackage{mdframed}

\usepackage{tikz}
\usepackage{authblk}

\usepackage[ruled,vlined,linesnumbered]{algorithm2e}

\newcommand{\nc}{\newcommand}
\nc{\rnc}{\renewcommand}

%\newcommand{\bra}[1]{\left\langle #1\right|}
%\newcommand{\ket}[1]{\left|#1\right\rangle}
\newcommand{\proj}[1]{\left|#1\right\rangle\left\langle #1\right|}
%\newcommand{\braket}[2]{\left\langle #1\middle|#2\right\rangle}
\newcommand{\vev}[1]{\left\langle #1\right\rangle}

\newcommand{\Rows}{\text{Rows}}
\newcommand{\Channel}{\text{Ch}}
\newcommand{\Coll}{\text{Coll}}
\newcommand{\Columns}{\text{Columns}}
\newcommand{\Haar}{\text{Haar}}
\newcommand{\lattice}{\text{lattice}}
\newcommand{\ie}{i.e.}
\newcommand{\tensor}{\otimes}
\newcommand{\ot}{\otimes}
\newcommand{\ad}{\mathrm{ad}}
\newcommand{\Id}{\mathrm{id}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\bigtensor}{\bigotimes}
\newcommand{\dist}{\mathsf{dist}}
\newcommand*{\vv}[1]{\vec{\mkern0mu#1}}
\newcommand{\multiprod}{\mathsf{multiprod}}
\newcommand{\vvec}{\mathsf{vec}}

\DeclareMathOperator{\abs}{abs}
\DeclareMathOperator{\Bin}{Bin}
\DeclareMathOperator{\conv}{conv}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\Img}{Im}
\DeclareMathOperator{\inj}{inj}
\DeclareMathOperator{\Par}{Par}
\DeclareMathOperator{\Pois}{\mathsf{Pois}}
\DeclareMathOperator{\poly}{poly}
\DeclareMathOperator{\polylog}{polylog}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\Sep}{Sep}
\DeclareMathOperator{\SepSym}{SepSym}
\DeclareMathOperator{\Span}{span}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\swap}{SWAP}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\ProdSym}{ProdSym}
\DeclareMathOperator{\SEP}{SEP}
\DeclareMathOperator{\PPT}{PPT}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Wg}{Wg}
\DeclareMathOperator{\WMEM}{WMEM}
\DeclareMathOperator{\WOPT}{WOPT}
\newcommand{\Tr}{\operatorname*{Tr}}

\DeclareMathOperator{\BPP}{\mathsf{BPP}}
\DeclareMathOperator{\FBPP}{\mathsf{FBPP}}
\renewcommand{\P}{\mathsf{P}}
\DeclareMathOperator{\BQP}{\mathsf{BQP}}
\DeclareMathOperator{\cnot}{\normalfont\textsc{cnot}}
\DeclareMathOperator{\DTIME}{\mathsf{DTIME}}
\DeclareMathOperator{\NTIME}{\mathsf{NTIME}}
\DeclareMathOperator{\MA}{\mathsf{MA}}
\DeclareMathOperator{\NP}{\mathsf{NP}}
\DeclareMathOperator{\coNP}{\mathsf{co-NP}}
\DeclareMathOperator{\PH}{\mathsf{PH}}
\DeclareMathOperator{\SharpP}{\mathsf{\#P}}
\DeclareMathOperator{\NEXP}{\mathsf{NEXP}}
\DeclareMathOperator{\Ptime}{\mathsf{P}}
\DeclareMathOperator{\QMA}{\mathsf{QMA}}
\DeclareMathOperator{\QCMA}{\mathsf{QCMA}}
\DeclareMathOperator{\BellQMA}{\mathsf{BellQMA}}
\DeclareMathOperator{\PostBPP}{\mathsf{PostBPP}}
\DeclareMathOperator{\PostBQP}{\mathsf{PostBQP}}

\def\sat{\text{3-SAT}}
\def\be#1\ee{\begin{equation}#1\end{equation}}
\def\bea#1\eea{\begin{eqnarray}#1\end{eqnarray}}
\def\beas#1\eeas{\begin{eqnarray*}#1\end{eqnarray*}}
\def\ba#1\ea{\begin{align}#1\end{align}}
\def\bas#1\eas{\begin{align*}#1\end{align*}}
\def\bpm#1\epm{\begin{pmatrix}#1\end{pmatrix}}
\nc{\non}{\nonumber}
\nc{\nn}{\nonumber}
\nc{\eq}[1]{(\ref{eq:#1})}
\nc{\eqs}[2]{(\ref{eq:#1}) and (\ref{eq:#2})}
%\def\eq#1{Eq.~(\ref{eq:#1})}
%\def\eqs#1#2{Eqs.~(\ref{eq:#1}) and (\ref{eq:#2})}
\rnc{\L}{\left} 
%\nc{\R}{\right}
\nc{\ra}{\rightarrow}
%\nc{\tensor}{\otimes}
\nc{\grad}{{\vec{\nabla}}}
%%%theorems
\newtheorem{theorem}{Theorem}
\newtheorem*{theorem*}{Theorem}
\newtheorem{remark}{Remark}
\newtheorem{conjecture}{Conjecture}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem*{lemma*}{Lemma}


\newtheorem{proposition}[theorem]{Proposition}
\newtheorem*{proposition*}{Proposition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem*{corollary*}{Corollary}
\newtheorem{problem}[theorem]{Problem}
\newenvironment{claim}[1]{\par\noindent \textbf{Claim:}\space#1}{}
\newenvironment{claimproof}[1]{\par\noindent{Proof:}\space#1}{\hfill $\blacksquare$}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{coupling}[theorem]{Coupling}
\newtheorem*{fact*}{Fact}

\nc\eps{\epsilon}

\def\vb{\vec{b}}
\def\vx{\vec{x}}
\def\Usch{U_{\text{Sch}}}

\nc\cA{\mathcal{A}}
\nc\cB{\mathcal{B}}
\nc\cC{\mathcal{C}}
\nc\cD{\mathcal{D}}
\nc\cE{\mathcal{E}}
\nc\cF{\mathcal{F}}
\nc\cG{\mathcal{G}}
\nc\cH{\mathcal{H}}
\nc\cI{\mathcal{I}}
\nc\cJ{\mathcal{J}}
\nc\cK{\mathcal{K}}
\nc\cL{\mathcal{L}}
\nc\cM{\mathcal{M}}
\nc\cN{\mathcal{N}}
\nc\cO{\mathcal{O}}
\nc\cP{\mathcal{P}}
\nc\cQ{\mathcal{Q}}
\nc\cR{\mathcal{R}}
\nc\cS{\mathcal{S}}
\nc\cT{\mathcal{T}}
\nc\cU{\mathcal{U}}
\nc\cV{\mathcal{V}}
\nc\cW{\mathcal{W}}
\nc\cX{\mathcal{X}}
\nc\cY{\mathcal{Y}}
\nc\cZ{\mathcal{Z}}

\def\bp{\mathbf{p}}
\def\bq{\mathbf{q}}
\def\bP{{\bf P}}
\def\bQ{{\bf Q}}
\def\gl{\mathfrak{gl}}

%\nc\bbC{\mathbb{C}}
%\nc\C{\mathbb{C}}
\DeclareMathOperator*{\E}{\mathbb{E}}
\DeclareMathOperator*{\bbE}{\mathbb{E}}
\nc\bbF{\mathbb{F}}
\nc\bbM{\mathbb{M}}
\nc\bbN{\mathbb{N}}
\nc\bbR{\mathbb{R}}
\nc\bbZ{\mathbb{Z}}
\newcommand{\Real}{\textrm{Re}}

\nc\benum{\begin{enumerate}}
\nc\eenum{\end{enumerate}}
\nc\bit{\begin{itemize}}
\nc\eit{\end{itemize}}
\newcommand{\fig}[1]{Fig.~\ref{fig:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\appref}[1]{Appendix~\ref{sec:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\propref}[1]{Proposition~\ref{prop:#1}}
\newcommand{\protoref}[1]{Protocol~\ref{proto:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\conref}[1]{Conjecture~\ref{con:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}

\newcommand{\FIXME}[1]{{\color{red}FIXME: #1}}
\nc{\todo}[1]{\textcolor{red}{todo: #1}}
\nc{\Anote}[1]{\textcolor{red}{Aram note: #1}}

\newcommand{\boxdfn}[2]{
\begin{figure}[h]\begin{center}
\noindent \framebox{\begin{minipage}{0.8\textwidth}
\begin{dfn}[{\bf #1}]\ \\ \\#2
\end{dfn}\end{minipage}}
\end{center}\end{figure}}

\newcommand{\boxproto}[2]{
\begin{figure}[h]\begin{center}
\noindent \framebox{\begin{minipage}{0.8\textwidth}
\begin{proto}[{\bf #1}]\ \\ \\#2\end{proto}
\end{minipage}}
\end{center}\end{figure}}

% FAIL
%\usepackage{environ}
%\newcounter{subeqcount}
%\NewEnviron{subeq}[1][subeq\addtocounter{subeqcount}{1}\arabic{subeqcount}]{%
%\begin{subequations}\label{eq:#1}\begin{align}\BODY\end{align}\end{subequations}}

\def\begsub#1#2\endsub{\begin{subequations}\label{eq:#1}\begin{align}#2\end{align}\end{subequations}}
\nc\qand{\qquad\text{and}\qquad}
\nc\mnb[1]{\medskip\noindent{\bf #1}}
\newcommand{\iso}[1]{\stackrel{#1}{\cong}}
\nc{\pder}[2]{\frac{\partial {#1}}{\partial {#2}}}
\nc{\p}{\partial}

==> New arXiv/restate.tex <==
% {{{ restate }}}
% set of macros to deal with restating theorem environments (or anything
% else with a label)

% stolen from Boaz's latex macros

% \MYstore{A}{B} assigns variable A value B
\newcommand{\MYstore}[2]{%
  \global\expandafter \def \csname MYMEMORY #1 \endcsname{#2}%
}

% \MYload{A} outputs value stored for variable A
\newcommand{\MYload}[1]{%
  \csname MYMEMORY #1 \endcsname%
}

% new label command, stores current label in \MYcurrentlabel
\newcommand{\MYnewlabel}[1]{%
  \newcommand\MYcurrentlabel{#1}%
  \MYoldlabel{#1}%
}

% new label command that doesn't do anything
\newcommand{\MYdummylabel}[1]{}

\newcommand{\torestate}[1]{%
  % overwrite label command
  \let\MYoldlabel\label%
  \let\label\MYnewlabel%
  #1%
  \MYstore{\MYcurrentlabel}{#1}%
  % restore old label command
  \let\label\MYoldlabel%
}

\newcommand{\restatetheorem}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{theorem*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{theorem*}
  \let\label\MYoldlabel
}

\newcommand{\restatelemma}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{lemma*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{lemma*}
  \let\label\MYoldlabel
}

\newcommand{\restateprop}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{proposition*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{proposition*}
  \let\label\MYoldlabel
}

\newcommand{\restatefact}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{fact*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{fact*}
  \let\label\MYoldlabel
}

\newcommand{\restatecorollary}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \begin{corollary*}[Restatement of \prettyref{#1}]
    \MYload{#1}
  \end{corollary*}
  \let\label\MYoldlabel
}

\newcommand{\restate}[1]{%
  % overwrite label command with dummy
  \let\MYoldlabel\label
  \let\label\MYdummylabel
  \MYload{#1}
  \let\label\MYoldlabel
}


==> Summary.tex <==
\begin{center}
%\begin{table}
\begin{tabular} 
%to 0.8\textwidth 
{ | c | c |}
 \hline
\textbf{Notation} & \textbf{Definition}\\
 \hline
 \hline
$\|\cdot \|_\diamond$ & super-operator diamond norm\\
\hline
$\|\cdot \|_p$ & matrix $p$-norm for $p \in [0, \infty]$\\
\hline
$\Haar$ & the Haar measure\\
\hline
$\Haar(S)$ & Haar measure on subset $S$ of qudits\\
\hline
$\Haar(i,j)$ & Haar measure on qudits $i$ and $j$\\
\hline
$r_{\alpha,i}$ & $i$-th row in the $\alpha$ direction\\
\hline 
$\text{Rows}(\alpha,n)$ & the collection of rows of a lattice (with $n$ points) in the $\alpha$ direction\\
\hline
$G^{(t)}_\mu$ & $t$-th order quasi-projector according to distribution $\mu$ over quantum circuits\\
\hline
$\braket{i,j| G^{(t)}_\mu|k,l}$ & balanced moment of order $t$ defined as $\E_{C\sim \mu} [C_{i_1, j_1} \ldots C_{i_t, j_t} C\ast_{i_1, j_1} \ldots C^\ast_{i_t, j_t}]$\\
\hline
$\text{Ch}[G^{(t)}_\mu]$ & moment super-operator corresponding to $G^{(t)}_\mu$ also equal to $\E_{C \sim \mu}  [\mathrm{ ad}_{C^{\tensor t}} ]$\\
\hline
$G^{(t)}_\Haar$ & Haar projector of order $t$\\
\hline
$G^{(t)}_{i,j}$ & Haar projector of order $t$ on qudit $i$ and $j$\\
\hline
$g_{\text{Rows}(\alpha,n)}$ &  one step of the random circuit applied in parallel to the rows in $\alpha$ direction\\
\hline
$g_{R} (g_C)$ &  one step of the random circuit applied in parallel to the rows (columns) of a $2$D lattice\\
\hline
$G_{\text{Rows}(\alpha,n)}$ &  Haar projector applied in parallel to the rows in $\alpha$ direction\\
\hline
$G_R(G_C)$ &  Haar projector applied in parallel to the rows (columns) of a $2$D lattice\\
\hline
$G_{\text{Planes}(\alpha)}$ & Haar projector applied in parallel to the plane that are perpendicular to the direction $\alpha$\\
\hline
$\text{Coll} (\cA)$ & collision probability from super-operator $\cA$\\
\hline
$\text{Coll}_s$ & the expected collision probability of a random circuit after $s$ steps \\
\hline
$\mu^{\lattice,n}_{D,c,s}$ & the distribution over $D$-dimensional random circuits with $n$ qidits and parameters $c,s$\\
\hline
$\mu^{\text{CG}}_{s}$ & the distribution over random circuits after application of $s$ random long range gates\\
\hline
${\tilde G}_{n,D,c}$ & same as $G^{(t)}_{\mu^{\lattice,n}_{D,c,s}}$ except that we replace $g^s_{\text{Rows} (\alpha,n)}$ with $G_{\text{Rows} (\alpha,n)}$.\\
\hline
${\hat G}_{n,D,c,s}$ & one block of ${\tilde G}_{n,D,c}$ defined as $G_{\text{Rows}(D,n)} \tilde{G}^{\tensor n^{1/D}}_{n^{1-1/D}, D-1, c,s} G_{\text{Rows}(D,n)}$.\\
\hline
\end{tabular}
%\caption{Summary of the notations and definitions used in this paper}
%\label{table:summary}
%\end{table}
\end{center}


==> circ2.tex <==
THIS FILE IS NO LONGER USED.  INSTEAD ITS BEEN MOVED TO CIRC1.TEX

\begin{figure}
\begin{center}
\begin{tikzpicture}[thick,scale=0.4]
\begin{scope}[rotate=90]

\foreach \y in {0,..., 5}{
\draw[blue] (0,\y) -- (1,\y); \draw[blue] (2,\y) -- (3,\y); \draw[blue] (4,\y) -- (5,\y); 
}

\foreach \x in {0,...,5}{
\foreach \y in {0,...,5}{
\fill [red] (\x,\y) circle (0.1);
}}


\foreach \x in {0,1,4,5}{
\foreach \y in {1,3,5}{
\fill[red] (\x,\y) circle (0.1);
}}
\foreach \y in {0,2,4}{
\fill[red] (2,\y) circle (0.1);
\fill[red] (3,\y) circle (0.1);
}


\node[inner sep=0,anchor=east,text width=1cm] (note1) at (2,8) {
   (2) };


\end{scope}


\begin{scope}[xshift=20cm]
\begin{scope}[rotate=90]

\foreach \y in {0,..., 5}{
\draw[blue] (1,\y) -- (2,\y); \draw[blue] (3,\y) -- (4,\y); 
}
\foreach \x in {0,...,5}{
\foreach \y in {0,...,5}{
\fill[red] (\x,\y) circle (0.1);
}}

\foreach \x in {0,1,4,5}{
\foreach \y in {1,3,5}{
\fill[red] (\x,\y) circle (0.1);
}}
\foreach \y in {0,2,4}{
\fill[red] (2,\y) circle (0.1);
\fill[red] (3,\y) circle (0.1);
}


\node[inner sep=0,anchor=east,text width=1cm] (note1) at (2,8) {
   (4) };

\end{scope}
\end{scope}
\end{tikzpicture}
\end{center}
\caption{ The random circuit model in definition \ref{def:modelsD}. Each red circle is a qudit and each blue link is a random $\text{SU}(d^2)$ gate. The model for $O(\sqrt n)$ first applies (1) and then (2). Then for $O(\sqrt n)$ first applies (3) and then (4), and continues these two steps for $O(1)$ rounds
%, and random single-qubit gates (red) are applied on other   qubits.
\label{fig:ourmodels}}
%\caption{ For $O(\sqrt n)$ time first apply (1) and then (2) and then for $O(\sqrt n)$ time first apply (3) and then (4) and repeat this for $O(1)$ times.\label{fig:google}}
\end{figure}
